Statistical biases in measurements with multiple candidates

Many measurements at collider experiments study physics candidates that are a subset of a collision event. The presence of multiple such candidates in a given event can cause raw biases which are large compared to typical statistical uncertainties. Selecting a single candidate is common practice but only helps if the likelihood of selecting the true candidate is very high. Otherwise the precision of the measurement can be affected, and biases can be generated, even if none are present in the data sample prior to this operation. This paper aims at describing the problem in a systematic way. It sets definitions, provides examples of potential biases using pseudoexperiments and gives recommendations.

==> selection.tex <==
\withSections{\section{Reconstruction and selection effects}\label{Sec:Selection}}{\vskip 1em}%
The candidate multiplicity usually decreases with more stringent selection
requirements.
Any multiple candidate removal procedure should thus be applied at the last stage,
once all the selection has been applied. If the candidate multiplicity is large 
in comparison to the precision of the measurement,
the selection criteria should be revisited. 
% If a correlation between the rate
% of multiple candidates and the particle multiplicity in the event is observed, 
% it is advised to consider vetoing large-multiplicity events. 
% Obviously, biases caused by this veto should be avoided, as
% in the case of a cross-section measurement.
The additional uncertainty due to this operation --- 
the uncertainty on this efficiency (see Section~\ref{Sec:Efficiencies})
as well as the increased relative statistical 
uncertainty due to the reduced signal yield --- has to be compared with the
systematic uncertainty related to the presence of multiple candidates.
Usually these uncertainties are not reported in publications.

A candidate arbitration is sometimes part of the design of the selection.
For instance the highest \pt lepton, or the most energetic jet may be used as seed to further reconstruction.
The subsequent comments on agreement between data and simulation, or signal and control channels,
also apply to such cases.
More generally, the particle trajectory reconstruction software --- known as pattern recognition --- 
applies arbitration by design~\cite{Fruhwirth:1987fm,pattern}. 
The tracking efficiency is calibrated using data~\cite{ATLAS:2012jma,Chatrchyan:2014fea,LHCb-DP-2013-002},
thus removing potential biases.



